Clover: Closed-Loop Verifiable Code Generation

The use of large language models for code generation is a rapidly growing trend in software development. However, without effective methods for ensuring the correctness of generated code, this trend could lead to undesirable outcomes. In this paper, we introduce a new approach for addressing this challenge: the Clover paradigm, short for Closed-Loop Verifiable Code Generation, which uses consistency checking to provide a strong filter for incorrect code. Clover performs consistency checks among code, docstrings, and formal annotations. The checker is implemented using a novel integration of formal verification tools and large language models. We provide a theoretical analysis to support our thesis that Clover should be effective at consistency checking. We also empirically investigate its performance on a hand-designed dataset (CloverBench) featuring annotated Dafny programs at a textbook level of difficulty. Experimental results show that for this dataset: (i) LLMs are reasonably successful at automatically generating formal specifications; and (ii) our consistency checker achieves a promising acceptance rate (up to 87%) for correct instances while maintaining zero tolerance for adversarial incorrect ones (no false positives). Clover also discovered 6 incorrect programs in the existing human-written dataset MBPP-DFY-50.

==> sec_analytical.tex <==
\section{An Analytical Model for \sys Reconstruction Tests}
\label{sec:clover_analytical}

As described above, all but one of the six Clover consistency checks relies on reconstructing one of the components (see Figure~\ref{fig:overview}).  These reconstructions rely on assumptions about the LLM model used for reconstruction that have, until now, been implicit.  In this section, we make these assumptions explicit and provide a theoretical model and analysis for those assumptions. 
For the purpose of the analysis we focus on a single directed edge from domain $A$ to domain $B$ (e.g., code to docstring).

Assume each domain is equipped with a semantic equivalence relation, denoted by $\equiv$.
Each domain can therefore be partitioned into equivalence classes.
For $X\in\{A,B\}$, we use $e(X)$ to denote the set of equivalence classes of $X$, and for $x \in X$ we use $[x]$ to denote the equivalence class $x$ belongs to.
For docstrings, the equivalence relation represents semantic equivalence as understood by a human expert; for code, the equivalence relation is functional equivalence; and for annotations, it is logical equivalence.

We further assume a \emph{ground truth consistency relation} between $A$ and $B$, denoted by $G \subseteq A \times B$. The ground truth consistency represents the consistency we assume to exist between docstrings, annotations, and code, as described in Section~\ref{sec:clover_schema}.
We assume the consistency relation satisfies the following properties that link it to the equivalence relation:
For any $x, x'\in A$ and $y, y' \in B$,
$(x \equiv x' \wedge y \equiv y') \rightarrow ((x, y) \in G \leftrightarrow (x', y')\in G)$ and
$((x, y) \in G \wedge (x', y')\in G) \rightarrow (x \equiv x' \leftrightarrow y \equiv y')$.
That is, consistency is preserved when substituting equivalent objects, and any object may be consistent with at most one equivalence class from the other domain.

We now formally define and analyze the \emph{single-edge \sys consistency test}, which aims to be an approximate test for $G$. For the analysis, we assume a probability distribution $\mathcal{D}$ on $A \times B$. The test relies on a \emph{transfer model} and the analysis assumes it is \emph{transfer-rational}, as defined below.

\begin{definition}[Transfer Model]
Given domains $A$ and $B$, a transfer model for $A$ and $B$ is a function $M: A\times B \rightarrow \mathbb{R}$
such that for each $x\in A$, $M(x, \cdot)$ is a probability distribution over $B$.
%(that is, $M(x, y)\ge 0$ for all $y\in B$ and $\sum_{y\in B}M(x, y)=1$).
Here $M(x, y)$ denotes the probability of transferring $x\in A$ to $y \in B$.
\end{definition}

\begin{definition}[Transfer-Rational Model]
Let $M$ be a transfer model for $A$ and $B$.
We say $M$ is \textit{transfer-rational} if for each $x\in A$ there is a unique $[y]\in e(B)$ that maximizes $\sum_{y'\in [y]} M(x, y')$.
In this case, we define the \textit{transfer function of} $M$,  $f^M: A \rightarrow e(B) = \lambda x. \, \argmax_{[y]\in e(B)} \sum_{y'\in [y]} M(x, y')$.


\end{definition}

Intuitively, the transfer model is meant to approximate a mapping based on the ground truth consistency ($G$).
In the context of \sys, the domains are among docstring, annotation, and code, and the transfer model is given by an LLM (\gpt). For example, when $A$ is docstrings and $B$ is annotations, the distribution $M(x, \cdot)$ represents the output distribution of \gpt on an input docstring $x$ with a suitable prompt for generating an annotation corresponding to the docstring $x$.
In our evaluation, we use 3 tries with \dafny feedback to run the reconstruction test.
In this case, the transfer model is given by this combined use of \gpt and \dafny.

We now fix a transfer-rational model $M$, and define the single-edge \sys consistency check.

\begin{definition}[Single-Edge \sys Consistency Check]
For input $x\in A, y\in B$, the single-edge \sys consistency check (for the edge from $A$ to $B$) is a procedure that draws $y'$ from the distribution $M(x,\cdot)$, and then accepts if $y' \equiv y$ and otherwise rejects.
\end{definition}

Note that the check relies on being able to check equivalence in domain $B$.\footnote{We assume a perfect equivalence check to keep the analysis simple and illustrative. In practice, the equivalence tests do incur some imprecision. But accounting for this imprecision using a probabilistic model is cumbersome because the distribution on the equivalence checks \sys performs depends on both the input distribution and on the transfer model.}

We now analyze the probability that the single-edge \sys consistency check is correct. Our analysis relies on two assumptions: one relating the transfer model $M$ with the ground truth consistency $G$, and another ensuring that $M$'s distributions are concentrated.

\begin{assumption}[Consistency Alignment]
\label{asmp:gtconsistency}
Let $c_1$ be the probability that $y\in f^M(x)$
when $x, y$ are sampled from $A\times B$ according to $\mathcal{D}$ conditioned on $(x, y)\in G$.
Similarly, let $c_0$ be the probability that $y\in f^M(x)$
when $x, y$ are sampled from $A\times B$ according to $\mathcal{D}$ conditioned on $(x, y)\not\in G$.
We assume that $c_1$ is close to 1, and $c_0$ is close to 0.
\end{assumption}

\begin{assumption}[Concentration]
\label{asmp:transfer-function}
Consider $x, y$ sampled from $A\times B$ according to $\mathcal{D}$
conditioned on $(x, y) \in G$ and $y\in f^M(x)$.
We assume that for some significant $0<l\leq 1$ (e.g., 30\%), the following holds with probability $\geq p_c$ ($p_c$ close to 1): 
$\sum_{y'\in f^M(x)} M(x, y') \geq l$.
%
Similarly, consider $x, y$ sampled from $A\times B$ according to $\mathcal{D}$
conditioned on $(x, y) \notin G$ and $y\notin f^M(x)$.
We assume that for some negligible $u$, the following holds with probability $\geq p_c$:
$\max_{[y_1]\in e(Y), [y_1]\neq f^M(x)} \sum_{y_2\in [y_1]} M(x, y_2)\leq u$.
\end{assumption}

Intuitively, the concentration assumption means that with high probability ($\geq p_c$), sampling from $M$ is the same as applying $f^M$, and specifically that the second most likely equivalence class is much less likely than the maximal one (i.e., the one given by $f^M$).

\begin{theorem}
\todo{why two assumptions point to same place}
\label{thm:clover}
Under Assumptions Consistency~\ref{asmp:gtconsistency} and Concentration~\ref{asmp:transfer-function}, 
consider $(x, y)$ sampled from $A\times B$ according to $\mathcal{D}$
conditioned on $(x, y)\in G$;
% \ben{It's not clear what it means to say "under Assumptions 3.4 and 3.5" since the assumptions involve vague terms like "non-negligible", "significantly smaller", and "close to". It seems there are two things that are being baked into the assumptions. One is a precise definition of variables like $c_1$, $c_0$, $p_c$, etc. The other is a vague assumption about the values of these probabilities. Maybe the theorem only depends on the definitions, in which case the definitions should be separated out from the assumptions. (If the theorem depends on the assumptions, then they need to be precise.)}
the single-edge \sys consistency check will accept $(x, y)$ with probability 
$A\geq l \cdot p_c \cdot c_1$.
Similarly, consider $(x, y)$ sampled from $A\times B$ according to $\mathcal{D}$ 
conditioned on $(x, y)\notin G$;
the single-edge \sys consistency check will 
will accept with probability $R \leq u \cdot p_c\cdot (1 - c_0) + (1-p_c)(1-c_0) + c_0$.
%
\end{theorem}

The proof of Theorem~\ref{thm:clover} is in Appendix~\ref{sec:appendix:proof}.

Theorem~\ref{thm:clover} ensures that under our assumptions, the probability of accepting a consistent input is significant, and the probability of accepting an inconsistent input is negligible. We can increase the gap by repeating the reconstruction test several times and accepting if any of them accept. 
% \ben{Maybe make precise what happens to the probability when you apply the procedure repeatedly. Does the chance of error go down exponentially?}
As discussed in Section~\ref{sec:evaluation}, our evaluation shows the results for both 1 and 10 reconstruction attempts.

\textbf{From single-edge to full \sys consistency checking.} Our analysis focused on a single, directed reconstruction edge from Figure~\ref{fig:overview}, while full \sys consistency checking uses five reconstruction edges and a single verification edge, and accepts only if all six checks accept. We do not attempt to theoretically analyze the full check, because we do not assume the edges to be independent (so multiplying acceptance probabilities is not necessarily meaningful). 
% \ben{Can anything be said from a theoretical perspective, possibly under some idealized assumptions? The failure of some variables to be independent does not mean that there is nothing that can be said, (e.g., see the Lovász local lemma).}
In our experiments, we empirically measure the acceptance rate of each edge, and also observe that the edges are not independent (see Section~\ref{sec:instantiation}).
In real experiments, the combined use of \gpt and \dafny may not satisfy our assumptions because of the tools' limitations (\dafny may time out or return unknown, and \gpt may make mistakes or hallucinate). Especially the $u$ in Assumption~\ref{asmp:transfer-function} could be non-negligible.
However, the end-to-end evaluation shows that the six checks together do give promising true positive and false positive rates.
The analytical model can be treated as one guide to understanding what properties of the reconstruction model are helpful for ensuring accurate reconstruction results.



==> sec_intro_backup.tex <==
\begin{abstract}


The use of large language models for code generation is a
rapidly growing trend in software development. 
However, without effective methods for ensuring the correctness of generated code, this trend could lead to undesirable outcomes. In this paper, we introduce a new tool for addressing this challenge: the \sys paradigm, short for \underline{Clo}sed-Loop \underline{Ver}ifiable Code Generation, which uses consistency checking to provide a strong filter for incorrect code. 
\sys performs consistency checks among code, docstrings, and formal annotations. The checker is implemented using a novel integration of formal verification tools and large language models. We provide a theoretical analysis to support our thesis that Clover should be effective at consistency checking. We also empirically investigate its performance on a hand-designed dataset (\dataset) featuring annotated \dafny programs at a textbook level of difficulty. Experimental results show that for this dataset, (i) LLMs are reasonably successful at automatically generating formal specifications; and (ii) our consistency checker achieves a promising acceptance rate (up to $87\%$) for correct instances while maintaining zero tolerance for incorrect ones (no false positives).
\end{abstract}

\section{Introduction}
\label{sec:intro}
Large language models (LLMs) have recently demonstrated remarkable capabilities.  They can engage in conversation, retrieve and summarize vast amounts of information, generate and explain text and code, and much more~\cite{bubeck2023sparks,DBLP:journals/corr/abs-2204-02311,DBLP:journals/corr/abs-2303-08774}. 
Among many possible applications, their ability to synthesize code based on natural language descriptions~\cite{DBLP:journals/corr/abs-2107-03374,DBLP:conf/iclr/ChengX0LNHXROZS23,li2022competition}
is stunning and could potentially enhance the productivity of programmers significantly~\cite{TN22}.  Indeed, futurists are already claiming that in the future, most code will be generated by LLMs (or their successors) and not by humans.

%\ying{Challenge:}
However, there is a fundamental challenge that must be overcome before realizing any version of this future. Currently, there is no trustworthy way to ensure the correctness of AI-generated code \cite{DBLP:journals/corr/abs-2305-01210}. Without some quality control, the prospect of dramatically scaling up code generation is highly concerning and could lead to catastrophic outcomes resulting from faulty code~\cite{DBLP:journals/corr/abs-2308-04451,DBLP:journals/corr/abs-2211-03622,DBLP:conf/uss/SandovalPNKGD23}.
For the most part, the current best practice for curating AI-generated artifacts is to have a human expert in the loop, e.g., \cite{copilot}.  While this is better than nothing, requiring human oversight of AI-generated code limits scalability.  Furthermore,
recent work \cite{hendler2023understanding,DBLP:conf/sp/PearceA0DK22,DBLP:conf/chi/Vaithilingam0G22,DBLP:journals/tosem/XuVN22} confirms the many risks and limitations of using AI even as a code assistant.
% \citet{DBLP:conf/sp/FischerBXSA0F17, DBLP:journals/tse/KrugerSABM21,DBLP:conf/uss/VotipkaFPHM020} investigate broadly existing security vulnerabilities in software,
Results suggest that developers with access to AI assistants write more insecure code, while at the same time having higher confidence in their code~\cite{DBLP:journals/corr/abs-2211-03622}.

It is becoming clear that curating the quality of AI-generated content will be one of the most crucial research challenges in the coming years. However, in the specific case of generated code, \emph{formal verification} can provide mathematically rigorous guarantees on the quality and correctness of code.  What if there were a way to \emph{automatically} apply formal verification to generated code?  This would not only provide a scalable solution, but it could actually lead to a future in which generated code is \emph{more reliable} than human-written code.

Currently, formal verification is only possible with the aid of time-consuming human expertise.  The main hypothesis of this paper is that \emph{LLMs are well-positioned to generate the collateral needed to help formal verification succeed}; furthermore, they can do this \emph{without compromising the formal guarantees provided by formal methods}.  To understand how, consider the following breakdown of formal verification into three parts: (i) construct a mathematical model of the system to be verified; (ii) provide a formal specification of what the system should do; and (iii) prove that the model satisfies the specification.
For code, step (i) is simply a matter of converting the code into mathematical logic, which can be done automatically based on the semantics of the programming language.  And step (iii) can often be done automatically thanks to powerful automated reasoning systems for Boolean satisfiability (SAT) and satisfiability modulo theories (SMT)~\cite{sathandbook}.  In fact, a number of tools already exist that take a specification (the result of step~(ii)) and some code as input and largely automate steps~(i) and (iii) (e.g., \cite{spark,lattuada2023verus,leino2010dafny}).\footnote{Such tools have plenty of room for improvement and must be extended to more mainstream languages, but separate research efforts are addressing this.}
% \CB{Add citation to Verus here}
%
However, step~(ii) appears to be a showstopper for automated formal verification of generated code, as traditionally, significant human expertise is required to create formal specifications and ensure that they are both internally consistent and accurately capture the intended functionality.

Two key insights suggest a way forward.  The first insight is simply a shift in perspective: the result of any AI-based code generation technique should aim to include \emph{not only code, but also formal specifications and natural language docstrings}.  The second insight is that given these components, we can use formal tools coupled with generative AI techniques to ensure that they are consistent.
We name our approach \emph{Clover}, short for \emph{Closed-loop Verifiable Code Generation}, and we predict that \sys, coupled with steadily improving generative AI and formal tools, will enable a future in which fully automatic, scalable generation of formally verified code is feasible. This paper charts the first steps towards realizing this vision.
%Here, we focus on the challenge of step (ii).\ying{Is this our focus?} \livia{yes since doc and code generation is already done but annotation generation is rare.}\todo{what we do does not help with formal if no LLM is introduced}\oded{I'm not sure saying that our focus is (ii) sets the right expectation for the rest of the paper. We don't provide a new technique for synthesizing formal specifications. I think maybe it's possible to remove everything from "For code, step (i)..." until the end of this paragraph and then join it with the following paragraph. Then, perhaps we can say something along the lines of: "The key challenge identified and addressed by this paper is ensuring consistency between code, docstring, and annotation, assuming that some (or even all) of the pieces are generated by AI." In other words, I suggest to first describe the more futuristic vision (as the next paragraph does) and only then present the focus of this paper.} Traditionally, significant human expertise is required to create formal specifications and ensure that they are both internally consistent and consistent with human expectations and understanding.



The \sys paradigm consists of two phases. 
In the first (generation) phase, some process is used to create code annotated with a formal specification and accompanied by a natural language documentation string (for simplicity, we refer to the latter two simply as ``annotations'' and ``docstrings'' going forward).  This could be a one-shot generative process in which a generative AI agent creates all three parts.  Alternatively, one or two of these components might already exist, in which case generative AI might be used to construct only the other(s).  In fact, the second phase is completely agnostic to the process used in the first phase; we simply insist that the result of the first phase has all three components: code, annotations, and docstrings.
In the second (verification) phase, a series of \emph{consistency checks} are applied to the code, annotations, and docstrings.  The Clover hypothesis is that if the consistency checks pass, then (i) the code is functionally correct with respect to its annotation; (ii) the annotation captures the full functionality of the code; and (iii) the docstring also accurately reflects the functionality of the code (see Figure~\ref{fig:overview}).

\begin{wrapfigure}{tr}{0.4\textwidth}
\vspace{-1.5em}
\includegraphics[width=0.4\textwidth]{figures/clover_overview.pdf}
\vspace{-2em}
\footnotesize \caption{The \sys paradigm}
\label{fig:overview}
\vspace{-0.5em}
\end{wrapfigure}



The idea is that we can unleash increasingly powerful and creative generative AI techniques in the generation phase, and then use the verification phase as a strong filter that only approves of code that is formally verified, accurately documented, and internally consistent.

In this paper, we focus on the verification phase, though we also include some demonstrations of the generation phase in our evaluation.  Our contributions include:
\begin{itemize}[topsep=0pt, leftmargin=16pt]
%\vspace{-0.3em}
    \item the Clover paradigm with a solution for the verification phase (Section~\ref{sec:clover_schema});
    \item the \dataset dataset, featuring manually annotated Dafny programs with docstrings, which contains both ground-truth examples and incorrect examples (Section~\ref{sec:dataset});
    % for empirically evaluating the consistency checking phase of \sys;
    \item a demonstration of the feasibility of using \gpt to generate code, specifications, and both (Section~\ref{sec:exp:generation});
    % \todo{not only specifications};
    \item implementation and evaluation of the verification phase of the \sys paradigm using \gpt and the Dafny verification tool (Section~\ref{sec:exp:ground_truth} and Section~\ref{sec:exp:inconsistency}).
    \item a theoretical framework which argues for the trustworthiness of the Clover approach (Section~\ref{sec:clover_analytical}); 
\end{itemize}

Our initial results on \dataset are promising.  Our implementation accepts $87\%$ of the correct examples and rejects $100\%$ of the incorrect examples.
We expect that the acceptance rate can be improved in a variety of ways while maintaining the strong ability to reject incorrect code.%
\footnote{The \dataset dataset and \sys consistency checking implementation will be made available after the anonymous review period.}
% \ying{why this?} \livia{delete?}}
%at \url{https://github.com/ChuyueSun/CLOVER}.

\begin{comment}   
Apart from the theoretical paradigm we developed as a foundation for future research in automatic AI-assisted verification, we also empirically investigate its practical feasibility by using \gpt together with a manually curated dataset (\dataset) featuring programs at a textbook-level difficulty.
Early experiments on \dataset are promising, with a $73\%$ acceptance rate for correct answers and a $100\%$ rejection rate for incorrect ones.
The dataset \dataset will be maintained and easily extesible. We envision the acceptance rate for correct answers grows as the model's capability improves.
\end{comment}




% \ying{Page plan:

% Sec 1 - Abstract and Intro: 1.5 page

% Sec 2 - Backgroud: 0.8 page

% Sec 3 - Clover: 3.5 pages

% Sec 4 - Dataset: 0.5 page

% Sec 5 - Evaluation: 2.5 pages

% Conclusion and ack: 0.2 page 
% }

==> tables/C1/C1_table.tex <==
\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & R  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & R  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & R  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & R  & R  & R  & R  & A  & A  \\ \hline
\end{tabular}}
    \caption{C1: If any one of the cells in a row is rejected, then the inconsistent example is successfully rejected. In this table, all examples are rejected.}
    \label{table:C1}
\end{table}



==> tables/C1/C1_table_k10.tex <==
\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & R  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & R  & A  & R  & A  &  A & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & R  & A  & R  & A  &  A & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & R  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & A  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & R  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & R  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & R  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & R  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & R  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & R  & R  & R  & R  & A  & A  \\ \hline
\end{tabular}}
    \caption{C1 when k=10}
    \label{table:C1_k10}
\end{table}



==> tables/C2/C2_table.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline

\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & A  & R  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & A  & R  & R  & A  & R  & R  \\ \hline
\end{tabular}}
    \caption{C2: all examples are rejected}
    \label{table:C2}
\end{table}



==> tables/C2/C2_table_k10.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline

\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & A  & R  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & A  & A  & R  & A  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  & R  & A  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & A  & R  & R  & A  & R  & R  \\ \hline
\end{tabular}}
    \caption{C2 when k=10}
    \label{table:C2_k10}
\end{table}



==> tables/C4/C4_table.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & R  & R  & A  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & A  & R  & R  & R  & A  & A  \\ \hline
\end{tabular}}
    \caption{C3: all examples are rejected}
    \label{table:C3}
\end{table}



==> tables/C4/C4_table_k10.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Row No. & test & anno-sound & anno-complete & doc2anno & doc2code & anno2doc & code2doc\\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  & R  & R  & R  &  A \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & A  & R  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & A  & R  & R  & R  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & R  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  & R  & R  & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & A  & R  & R  & R  & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & R  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & A  & R  & A  & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & A  & A  & R  & R  & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & A  & R  & R  & R  & A  & A  \\ \hline
\end{tabular}}
    \caption{C3 when =10 }
    \label{table:C3_k10}
\end{table}



==> tables/anno2code/anno2code_noverify.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & f \\ \hline
\end{tabular}
    \caption{anno2code}
    \label{table:anno2code}
\end{table}



==> tables/anno2code/anno2code_onetry.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & f \\ \hline
\end{tabular}
    \caption{anno2code}
    \label{table:anno2code}
\end{table}



==> tables/anno2code/anno2code_table.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & f \\ \hline
\end{tabular}
    \caption{anno2code}
    \label{table:anno2code}
\end{table}



==> tables/anno2code/claude.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & f \\ \hline

\end{tabular}
    \caption{anno2code}
    \label{table:anno2code}
\end{table}



==> tables/anno2code/table_individual_task.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & abs & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_append & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_concat & f \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_copy & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  array\_product & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_sum & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  avg & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  binary\_search & f:need to strength \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & bubble\_sort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_ans & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_sum & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   canyon\_search & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  compare & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  convert\_map\_key & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  count\_less\_than & f \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   double\_quadruple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & even\_list & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  find & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  integer\_square\_root & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  is\_even & eq \\ \hline

   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search1 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search3 & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   longest\_prefix & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  max\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_of\_2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  modify\_2d\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  multi\_return & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & online\_max & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  only\_once & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  quotient & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  remove\_front & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  return\_seven & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  rotate & f \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   selectionsort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_array & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_seq & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  slope\_search & f:need to strength \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & swap\_arith & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   swap\_bitvector & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_in\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_sim & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  test\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple3 & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple4 & eq \\ \hline
       \stepcounter{rowcount}\arabic{rowcount} &  update\_array & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & update\_map & f \\ \hline

\end{tabular}
    \caption{anno2code}
    \label{table:anno2code}
\end{table}



==> tables/anno2doc/anno2doc.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & abs & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_append & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_concat & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_copy & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  array\_product & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_sum & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  avg & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  binary\_search & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & bubble\_sort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_ans & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_sum & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   canyon\_search & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  compare & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  convert\_map\_key & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  count\_less\_than & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   double\_quadruple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & even\_list & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  find & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  integer\_square\_root & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  is\_even & eq \\ \hline

   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search1 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search3 & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   longest\_prefix & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  max\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_of\_2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  modify\_2d\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  multi\_return & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & online\_max & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  only\_once & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  quotient & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  remove\_front & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  replace & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  return\_seven & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  rotate & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   selectionsort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  seq\_to\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_seq & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  slope\_search & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & swap\_arith & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   swap\_bitvector & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_in\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_sim & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  test\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple3 & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple4 & eq \\ \hline
       \stepcounter{rowcount}\arabic{rowcount} &  update\_array & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & update\_map & eq \\ \hline

\end{tabular}
    \caption{anno2doc}
    \label{table:anno2doc}
\end{table}



==> tables/code2anno/code2anno_CLOVER.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \resizebox{0.58\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|}
    \hline
    Row No. & test & normal & random\_mutation \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &all\_digits & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &below\_zero & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &copy\_part & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &has\_close\_elements & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &insert & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_palindrome & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & R  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &reverse & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & R  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &two\_sum & A  & R  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & A  & A  \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & R  & R  \\ \hline
\end{tabular}}
    \caption{Ablation studies for random mutation in annotation generation}
    \label{table:code2anno_clover}
\end{table}



==> tables/code2doc/code2doc.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & abs & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_append & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_concat & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_copy & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  array\_product & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_sum & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  avg & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  binary\_search & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & bubble\_sort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_ans & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_sum & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   canyon\_search & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  compare & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  convert\_map\_key & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  count\_less\_than & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   double\_quadruple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & even\_list & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  find & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  integer\_square\_root & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  is\_even & eq \\ \hline

   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search1 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search3 & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   longest\_prefix & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  max\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_of\_2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  modify\_2d\_array & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  multi\_return & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & online\_max & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  only\_once & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  quotient & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  remove\_front & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  replace & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  return\_seven & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  rotate & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   selectionsort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  seq\_to\_array & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_seq & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  slope\_search & f \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & swap\_arith & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   swap\_bitvector & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_in\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_sim & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  test\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple3 & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple4 & eq \\ \hline
       \stepcounter{rowcount}\arabic{rowcount} &  update\_array & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & update\_map & eq \\ \hline

\end{tabular}
    \caption{code2doc}
    \label{table:code2doc}
\end{table}



==> tables/doc2anno/doc2anno_noVerify.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & abs & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_append & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_concat & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_copy & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  array\_product & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_sum & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  avg & f:stronger gen pre \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  binary\_search & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & bubble\_sort & f: weaker gen post \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_ans & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_sum & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   canyon\_search & f: weaker gen post \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  compare & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  convert\_map\_key & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  count\_less\_than & f \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   double\_quadruple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & even\_list & f: weaker gen pre \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  find & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  integer\_square\_root & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  is\_even & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search1 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search3 & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   longest\_prefix & f: inaccurate gen post \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  max\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_of\_2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  modify\_2d\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  multi\_return & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & online\_max & f: syntax \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  only\_once & eq: cannot be auto verified \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  quotient & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  remove\_front & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  return\_seven & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  rotate & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   selectionsort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_seq & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  slope\_search & f:syntax \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & swap\_arith & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   swap\_bitvector & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_in\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_sim & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  test\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple3 & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple4 & eq \\ \hline
       \stepcounter{rowcount}\arabic{rowcount} &  update\_array & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & update\_map & f: weaker gen post\\ \hline

\end{tabular}
    \caption{doc2anno\_noVerify}
    \label{table:doc2anno_noverify}
\end{table}


==> tables/doc2anno/doc2anno_table.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & abs & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_append & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_concat & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_copy & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  array\_product & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & array\_sum & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  avg & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  binary\_search & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & bubble\_sort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_ans & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  cal\_sum & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   canyon\_search & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  compare & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  convert\_map\_key & f:cannot auto\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  count\_less\_than & f \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   double\_quadruple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & even\_list & f: weaker gen pre \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  find & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  integer\_square\_root & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  is\_even & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search1 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  linear\_search3 & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   longest\_prefix & f: inaccurate gen post \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  max\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  min\_of\_2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  modify\_2d\_array & f: syntax \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  multi\_return & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & online\_max & f: syntax \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  only\_once & f: cannot be auto verified \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  quotient & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  remove\_front & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  replace & eq \\ \hline

   \stepcounter{rowcount}\arabic{rowcount} &  return\_seven & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  rotate & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   selectionsort & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  set\_to\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  seq\_to\_seq & eq\\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  slope\_search & f:syntax \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & swap\_arith & eq \\ \hline
  \stepcounter{rowcount}\arabic{rowcount} &   swap\_bitvector & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_in\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  swap\_sim & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  test\_array & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple2 & eq \\ \hline
   \stepcounter{rowcount}\arabic{rowcount} &  triple3 & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & triple4 & eq \\ \hline
       \stepcounter{rowcount}\arabic{rowcount} &  update\_array & eq \\ \hline
    \stepcounter{rowcount}\arabic{rowcount} & update\_map & f: weaker gen post\\ \hline

\end{tabular}
    \caption{doc2anno}
    \label{table:doc2anno}
\end{table}



==> tables/doc2code/doc2code.tex <==

\begin{table}
    \centering
    \setcounter{rowcount}{0}
    \begin{tabular}{|c|c|c|}
    \hline
    Row No. & test & result \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &abs & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_append & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_concat & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_copy & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_product & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &array\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &avg & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &binary\_search & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &bubble\_sort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_ans & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &cal\_sum & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &canyon\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &compare & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &convert\_map\_key & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &count\_lessthan & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &double\_quadruple & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &even\_list & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &find & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &integer\_square\_root & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &is\_even & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search1 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &linear\_search3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &longest\_prefix & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &max\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &min\_of\_two & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &modify\_2d\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &multi\_return & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &online\_max & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &only\_once & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &quotient & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &remove\_front & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &replace & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &return\_seven & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &rotate & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &selectionsort & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &seq\_to\_array & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &set\_to\_seq & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &slope\_search & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap & f \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_arith & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_bitvector & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_in\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &swap\_sim & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &test\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple2 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple3 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &triple4 & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_array & eq \\ \hline
\stepcounter{rowcount}\arabic{rowcount} &update\_map & f \\ \hline
\end{tabular}
    \caption{doc2code}
    \label{table:doc2code}
\end{table}


